Efficient Training of Large Language Models on Distributed Infrastructures: A Survey

Large Language Models (LLMs) like GPT and LLaMA are revolutionizing the AI industry with their sophisticated capabilities. Training these models requires vast GPU clusters and significant computing time, posing major challenges in terms of scalability, efficiency, and reliability. This survey explores recent advancements in training systems for LLMs, including innovations in training infrastructure with AI accelerators, networking, storage, and scheduling. Additionally, the survey covers parallelism strategies, as well as optimizations for computation, communication, and memory in distributed LLM training. It also includes approaches of maintaining system reliability over extended training periods. By examining current innovations and future directions, this survey aims to provide valuable insights towards improving LLM training systems and tackling ongoing challenges. Furthermore, traditional digital circuit-based computing systems face significant constraints in meeting the computational demands of LLMs, highlighting the need for innovative solutions such as optical computing and optical networks.

==> contents/5_storage.tex <==
\section{Storage Optimizations}
\label{sec:storage} 

\subsection{Checkpoint Optimization}

Model checkpoints present a significant challenge to storage due to the continually increasing number of model parameters. The growing costs associated with model checkpoints cannot be overlooked, yet they remain an unavoidable component of fault-tolerant training. Currently, the community primarily focuses on two optimization goals: checkpoint frequency and asynchronous checkpoints.

\phb{Checkpoint Frequency.}

The storage frequency of model checkpoints essentially involves a trade-off. If the frequency is too low, a significant number of training steps can be wasted following an unexpected interruption in training; conversely, if the frequency is too high, it can place considerable strain on storage resources. CheckFreq\cite{mohan2021checkfreq} employs a systematic online analysis to find the right balance between recovery costs and runtime overhead. Specifically, CheckFreq determines the appropriate checkpoint frequency based on a user-provided tolerance for checkpoint overhead. Meanwhile, Gupta et al.\cite{gupta2024just} have proposed Just-In-Time Checkpointing, which calculates the optimal checkpoint interval based on the expected number of failures during a training period and the cost of performing a checkpoint, taking into account the actual duration of training and the conditions of the training hardware.

\phb{Asynchronous Checkpointing.}

==> figures/fig-tree-resource-efficient-architectures.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.5pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-red!10, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[htpb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=black,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={black, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=12em,font=\normalsize,}{},
            where level=2{text width=12em,font=\normalsize,}{},
            [
                \textbf{Resource-efficient Architecture}, ver
                        [
                          \textbf{Efficient Attention}, fill=blue!10
                          [
                          \textbf{Sparse Attention}, fill=yellow!10
                          [
                          Longformer~\cite{beltagy2020longformer}{, }
                          ETC~\cite{ainslie2020etc}{, }
                          BIGBIRD~\cite{zaheer2020big}{, }
                          HEPOS~\cite{huang2021efficient}{, }\\
                          MATE~\cite{eisenschlos2021mate}{, }
                          LittleBird~\cite{lee2022littlebird}{, }
                          ALBERT~\cite{lan2019albert}{, } 
                          TDANet~\cite{li2022efficient},
                          leaf, 
                          text width= 33em
                          ]
                          ]
                          [
                          \textbf{Approximate Attention}, fill=yellow!10
                          [
                          Reformer~\cite{kitaev2019reformer}{, }
                          Transformers are rnns~\cite{katharopoulos2020transformers}{, }
                          Linformer~\cite{wang2020linformer}{, }\\
                          Performers~\cite{choromanski2020rethinking}{, }
                          Luna~\cite{ma2021luna}{, }
                          Mega~\cite{ma2022mega}{, }\\
                          Deformable Attention~\cite{xia2022vision}{, }
                          CrossViT~\cite{chen2021crossvit}{, }
                          PolySketchFormer~\cite{kacham2023polysketchformer},
                          leaf, text width=33em
                          ]
                          ]
                          [
                          \textbf{Attention-Free Approaches}, fill=yellow!10
                          [
                          AFT~\cite{zhai2021attention}{, }
                          Perceiver~\cite{jaegle2021perceiver}{, }
                          Hyena hierarchy~\cite{poli2023hyena}{, }
                          RMT~\cite{bulatov2022recurrent, bulatov2023scaling}{, } \\
                          State space model (SSM)~\cite{gu2022efficiently, dao2022hungry, orvieto2023resurrecting, gu2023mamba}{, }
                          RWKV~\cite{peng2023rwkv}{, }
                          RetNet~\cite{sun2023retentive},
                          leaf, text width=33em
                          ]
                          ]
                        ]
                        [
                          \textbf{Dynamic Neural Network}, fill=blue!10 
                          [
                          \textbf{Mixture-of-Expert}, fill=yellow!10
                          [
                          Switch transformer~\cite{fedus2022switch}{, }
                          V-MoE~\cite{riquelme2021scaling}{, }
                          GLaM~\cite{du2022glam}{, }
                          LIMoE~\cite{mustafa2022multimodal}{, }\\
                          Mistral~\cite{jiang2023mistral}{, }
                          FFF~\cite{belcak2023fast}
                          MoEfication~\cite{zhang2022moefication}{, }
                          Sparse Upcycling~\cite{komatsuzaki2023sparse},
                          leaf, text width=33em
                          ]
                          ]
                          [
                          \textbf{Early-exiting}, fill=yellow!10
                          [
                          Simplifying transformer blocks~\cite{he2023simplifying}{, }
                          FREE~\cite{bae2023fast}{, }
                          PABEE~\cite{zhou2020bert}{, }\\
                          DeeBERT~\cite{xin2020deebert}{, }
                          LGViT~\cite{xu2023lgvit}{, }
                          Bakhtiarnia et al.\cite{bakhtiarnia2021multi}{, }
                          SkipDecode~\cite{del2023skipdecode},
                          leaf, text width=33em
                          ]
                          ]
                        ] 
                        [
                          \textbf{Diffusion-specific}\\ \textbf{~~~Optimization}, fill=blue!10 
                          [
                          \textbf{Efficient Sampling}, fill=yellow!10
                          [
                          iDDPM~\cite{nichol2021improved}{, }
                          DDIM~\cite{song2020denoising}{, }
                          PNDM~\cite{liu2022pseudo}{, }
                          DPM-Solver~\cite{lu2022dpm},
                          leaf, text width=33em
                          ]
                          ]
                          [
                          \textbf{Diffusion in Latent Space}, fill=yellow!10
                          [
                          LDM~\cite{rombach2022high}{, }
                          LD-ZNet~\cite{pnvr2023ld}{, }
                          SALAD~\cite{koo2023salad}{, }
                          Takagi et al.~\cite{takagi2023high},
                          leaf, text width=33em
                          ]
                          ]
                          [
                          \textbf{Diffusion Architecture}\\
                          \textbf{~~~~~~~~~~Variants}
                          , fill=yellow!10
                          [
                          SnapFusion~\cite{li2023snapfusion}{, }
                          ERNIE-ViLG~\cite{feng2023ernie}{, }
                          ScaleCrafter~\cite{he2023scalecrafter},
                          leaf, text width=33em
                          ]
                          ]
                        ]  
                        [
                          \textbf{ViT-specific Optimizations}, fill=blue!10 
                          [
                          LeViT~\cite{graham2021levit}{, } PoolFormer~\cite{yu2022metaformer}{, } MobileViT~\cite{mehta2022mobilevit}{, } EfficientFormer~\cite{li2022efficientformer}{, } 
                          EfficientViT~\cite{cai2022efficientvit},
                          leaf, text width=40em 
                          ]
                        ] 
                    ]
        \end{forest}
    }
    
    \caption{An overview of resource-efficient architectures.}
    \label{fig:tree-resource-efficient architecture tree}
\end{figure*}

==> figures/taxonomy_0_overall.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=black,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-red!10, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[htpb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
        forked edges,
        for tree={
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,
            child anchor=west,
            base=center,
            font=\large,
            rectangle,
            draw=black,
            rounded corners,
            align=left,
            text centered,
            minimum width=4em,
            edge+={black, line width=1pt},
            s sep=3pt,
            inner xsep=2pt,
            inner ysep=3pt,
            line width=0.8pt,
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
        },
        where level=1{text width=17em,font=\normalsize,}{},
        where level=2{text width=17em,font=\normalsize,}{},
        where level=3{text width=25em,font=\normalsize,}{},
        [
        {Efficient Distributed LLM Training}, ver 
                [
                {Infrastructure (\S \ref{sec:infra})}, fill=blue!10
                    [
                    {AI Accelerators (\S \ref{subsec:accelerators})}, fill=yellow!10
                        [
                        {NVIDIA GPU (\S \ref{subsubsec:gpu})}\\
                        {Other AI Accelerators (\S \ref{subsubsec:OtherAIAccelerators})},
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Network Infrastructure (\S \ref{subsec:networkinfra})}, fill=yellow!10
                        [
                        {Chip-to-Chip Communication (\S \ref{subsubsec:chip-to-chip})} \\            {Node-to-Node Communication (\S \ref{subsubsec:node-to-node})} \\
                        {Network Topology (\S \ref{subsubsec:topology})} \\
                        {Load Balancing \& Congestion Control (\S \ref{subsubsec:lbandcc})}, 
                        leaf, text width=25em
                        ]
                    ]
                ] 
                %%
                [
                {Parallelism Schemes (\S \ref{sec:parallel})}, fill=blue!10
                    [
                    {Hybrid Parallelism (\S \ref{subsec_hybrid_parallelism})}, fill=yellow!10
                        [
                        {Data Parallelism (\S \ref{subsubsec_data_parallelism})} \\
                        {Tensor Parallelism (\S \ref{subsubsec_tensor_parallelism})} \\
                        {Pipeline Parallelism (\S \ref{subsubsec_pipeline_parallelism})} \\
                        {Sequence Parallelism (\S \ref{subsubsec:SequenceParallelism})} \\
                        {Expert Parallelism (\S \ref{subsubsec:ExpertParallelism})},
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Auto Parallelism (\S \ref{subsec:AutoParallelism})}, fill=yellow!10
                        [
                        {General Framework (\S \ref{subsubsec:GeneralFramework})} \\
                        {Transformer Specific Framework (\S \ref{subsubsec:TransformerSpecificFramework})},
                        leaf, text width=25em
                        ]
                    ]
                    [
                    {Heterogeneous Parallelism (\S \ref{subsec:HeterogeneousParallelism})}, fill=yellow!10
                        [
                        {Heterogeneous Hardware (\S \ref{subsubsec:HeterogeneousHardware})} \\
                        {Heterogeneous Model (\S \ref{subsubsec:HeterogeneousModel})},
                        leaf, text width=25em
                        ]
                    ]
                ]           [
                {Computation Optimizations (\S \ref{sec:comp})}, fill=blue!10
                    [
                    {Operator Optimizations (\S \ref{subsec:OperatorOptimizations})}, fill=yellow!10
                        [
                        {Manually Optimizations (\S \ref{subsubsec:ManuallyOptimizedAttentionOperator})}\\
                        {Automatic Optimizations (\S \ref{subsubsec:AutomaticOptimizationsviaCompilers})}, 
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Mixed-precision Training (\S \ref{subsec:Mixed-precisionTraining})}, fill=yellow!10
                        [
                        {16-bit Floating Point  (\S \ref{subsubsec:16-BitFloatingPoint})} \\
                        {Sub-8-bit Floating Point  (\S \ref{subsubsec:8-BitFloatingPoint})} \\
                        {Low-bit Fixed Point (\S \ref{subsubsec:Low-BitFixedPoint})}, 
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {In-Network Aggregation (\S \ref{in-network})}, fill=yellow!10
                        [
                        {Ethernet-based Aggregation (\S \ref{ethernet-based})} \\
                        {Infiniband-based Aggregation (\S \ref{infiniband-based})}, 
                        leaf, text width=25em
                        ]
                    ]
                ] 
                %%
                [
                {Memory Optimizations (\S \ref{sec:mem})}, fill=blue!10
                    [
                    {Activation Recomputation (\S \ref{subsec_activation_recomputation})}, fill=yellow!10
                        [
                        {Static Evicting (\S \ref{subsubsec_static_evicting})} \\
                        {Dynamic Evicting (\S \ref{subsubsec_dynamic_evicting})},
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Redundancy Reduction (\S \ref{subsec_redundancy_reduction})}, fill=yellow!10
                        [
                        {Fully Sharding (\S \ref{subsubsec_full_sharding})} \\                        {Partially Sharding (\S \ref{subsubsec_partially_sharding})}, 
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Defragmentation (\S \ref{subsec_defragmentation})}, fill=yellow!10
                        [
                        {Tensor-based Defragmentation (\S \ref{subsubsec_tensor_based_defrag})}\\
                        {VMM-based Defragmentation (\S \ref{subsubsec_vmm_defrag})}, leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Offloading (\S \ref{subsec_offloading})}, fill=yellow!10
                        [
                        {CPU Offloading (\S \ref{subsubsec_cpu_offloading})}\\
                        {SSD Offloading (\S \ref{subsubsec_ssd_offloading})}, 
                        leaf, text width=25em
                        ]
                    ]
                ] 
                %%
                [
                {Communication Optimizations (\S \ref{sec:comm})}, fill=blue!10
                    [
                    {Collective Communication (\S \ref{collective_communication})}, fill=yellow!10
                        [
                        {Pre-Defined Algorithm (\S \ref{pre-defined})}\\
                        {Synthesized Algorithm (\S \ref{synthesized})}, 
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Communication Scheduling (\S \ref{communication-scheduling})}, fill=yellow!10
                        [
                        {FIFO-based Scheduling (\S \ref{fifo-based})} \\
                        {Priority-based Scheduling (\S \ref{priority-base})} \\
                        {Decomposition-based Scheduling (\S \ref{decomposition-based})}, 
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {In-Network Aggregation (\S \ref{in-network})}, fill=yellow!10
                        [
                        {Ethernet-based Aggregation (\S \ref{ethernet-based})} \\
                        {Infiniband-based Aggregation (\S \ref{infiniband-based})}, 
                        leaf, text width=25em
                        ]
                    ]
                ] 
                [
                {Fault Tolerance (\S \ref{sec:resi})}, fill=blue!10
                    [
                    {Anomaly Detection (\S \ref{subsec:AnomalyDetection})}, fill=yellow!10
                        [
                        {Statistical Monitoring (\S \ref{subsubsec:StatisticalMonitoring})}\\
                        {Proactive Validation (\S \ref{subsubsec:ProactiveValidation})}, 
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Checkpoint-Based Recovery (\S \ref{subsection:Checkpoint-basedRecovery})}, fill=yellow!10
                        [
                        {Persistent Checkpointing (\S \ref{subsection:PersistentCheckpoint})} \\
                        {In-Memory Checkpointing (\S \ref{subsubsection:In-MemoryCheckpointing})}, 
                        leaf, text width=25em
                        ]
                    ]
                    %%
                    [
                    {Checkpoint-Free Recovery (\S \ref{subsection:Checkpoint-FreeRecovery})}, fill=yellow!10
                        [
                        {Live Migration (\S \ref{subsubsection:Live-Migration})} \\
                        {Module Redundancy (\S \ref{subsubsection:Module-Redundancy})}, 
                        leaf, text width=25em
                        ]
                    ]
                ] 
        ]
        \end{forest}
    }
    
    \caption{The overall structure of this survey.}
    \label{taxonomy:overall}
\end{figure*}




==> figures/taxonomy_7_workloads.tex <==
\begin{figure*}[htpb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
        forked edges,
        for tree={
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,
            child anchor=west,
            base=center,
            font=\large,
            rectangle,
            draw=black,
            rounded corners,
            align=left,
            text centered,
            minimum width=4em,
            edge+={black, line width=1pt},
            s sep=3pt,
            inner xsep=2pt,
            inner ysep=3pt,
            line width=0.8pt,
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
        },
        where level=1{text width=12em,font=\normalsize,}{},
        where level=2{text width=14em,font=\normalsize,}{},
        [
        \textbf{Emerging Workloads}, ver
                [
                \textbf{MoE}, fill=blue!10
                    [
                    \textbf{Expert Parallelism}, fill=yellow!10
                        [
                        Gshard\cite{lepikhin2020gshard}{, }
                        Switch transformer\cite{fedus2022switch}{, }\\
                        Deepspeed-MoE\cite{rajbhandari2022deepspeed}{, }
                        Tutel\cite{hwang2023tutel},
                        leaf, 
                        text width= 31em
                        ]
                    ]
                    % 
                    [
                    \textbf{Computation Efficient}, fill=yellow!10
                        [
                        Megablock\cite{gale2023megablocks}{, }
                        ScatterMoE\cite{tan2024scattered}{, }
                        Tutel\cite{hwang2023tutel}{, }\\
                        FastMoE\cite{he2021fastmoe}{, }
                        PipeMoE\cite{shi2023pipemoe}{, }
                        ScheMoE\cite{shi2024schemoe}{, }\\
                        Lina\cite{li2023accelerating}{, }
                        Janus\cite{liu2023janus}{, }
                        TA-MoE\cite{chen2022ta},
                        leaf, 
                        text width= 31em
                        ]
                    ]
                    %
                    [
                    \textbf{Memory Efficient}, fill=yellow!10
                        [
                        MoESys\cite{yu2024moesys, shen2022se}{, }
                        MPipeMoE\cite{zhang2024mpmoe}{, }
                        M6-10T\cite{lin2021m6},
                        leaf, 
                        text width= 31em
                        ]
                    ]
                    %
                    [
                    \textbf{Load Balance}, fill=yellow!10
                        [
                        FasterMoE\cite{he2022fastermoe}{, }
                        SmartMoE\cite{zhai2023smartmoe}{, }
                        FlexMoE\cite{nie2023flexmoe}{, }
                        Prophet\cite{wang2023prophet},
                        leaf, 
                        text width= 31em
                        ]
                    ]
                ]
                %%
                [
                \textbf{Fine-Tuning}, fill=blue!10
                    [
                    \textbf{PEFT}, fill=yellow!10
                        [
                        LoRA\cite{hu2021lora}{, }
                        LLM-Adaptor\cite{hu2023llmadaptor}{, }
                        IA${}^3$\cite{liu2022ia3}{, }
                        Prefix-Tuning\cite{li2021prefixtuning}{, }\\
                        Prompt-Tuning\cite{lester2021prompttuning},
                        leaf, 
                        text width= 31em
                        ]
                    ]
                    % 
                    [
                    \textbf{MEFT}, fill=yellow!10
                        [
                        LOMO\cite{lv2023lomo}{, }
                        MeZO\cite{malladi2023mezo}{, }
                        QLoRA\cite{dettmers2023qlora}{, }
                        LISA~\cite{pan2024lisa}
                        ,
                        leaf, 
                        text width= 31em
                        ]
                    ]
                    %
                    [
                    \textbf{RLHF}, fill=yellow!10
                        [
                        DeepSpeed-Chat\cite{yao2023DeepSpeedChatEasy}{, }
                        DPO~\cite{rafailov2023DirectPreference}
                        ,
                        leaf, 
                        text width= 31em
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{An Overview of Communication Optimization Techniques.}
    \label{taxonomy:workloads}
\end{figure*}
